NavTuner: Learning a Scene-Sensitive Family of Navigation Policies

The advent of deep learning has inspired research into end-to-end learning for a variety of problem domains in robotics. For navigation, the resulting methods may not have the generalization properties desired let alone match the performance of traditional methods. Instead of learning a navigation policy, we explore learning an adaptive policy in the parameter space of an existing navigation module. Having adaptive parameters provides the navigation module with a family of policies that can be dynamically reconfigured based on the local scene structure, and addresses the common assertion in machine learning that engineered solutions are inflexible. Of the methods tested, reinforcement learning (RL) is shown to provide a significant performance boost to a modern navigation method through reduced sensitivity of its success rate to environmental clutter. The outcomes indicate that RL as a meta-policy learner, or dynamic parameter tuner, effectively robustifies algorithms sensitive to external, measurable nuisance factors.

==> approach.tex <==
Suppose we have an agent trying to navigate from its start pose $p_s$ to
its goal pose $p_g$ with a known map of the world. A global costmap
$M_{global}$, where the value of point $(x,y)$, $V_{x,y}$, is the cost
for the robot to travel to $(x,y)$, will be computed from the known map.
The cost for unnavigable points, such as points occupied by objects or
obstacles, will be higher, while cost for collision-free points will be
lower. Upon receiving $p_g$, the global planner will generate a global
path $P_{global}$ from $p_s$ to $p_g$ based on $M_{global}$, and send it
to the local planner $L_\theta$ whose hyper-parameters are $\theta$. The
agent will be controlled by $L_\theta$. During the navigation, a local
costmap $M_{local}$ will be computed from the robot's sensor data, such
as depth map or laserscan. $L_\theta$ will take in $P_{global}$ and
$M_{local}$, and generate a local path $P_{local}$, which will be sent
to the robot as velocity commands. $M_{global}$, $P_{global}$, and
$P_{local}$ will be updated at certain frequencies $f_{MG}$, $f_{PG}$,
and $f_{PL}$ respectively. Suppose we have a evaluation function
$h(L_\theta)$ that will give a higher score to local planner with better
performance. We are trying to build a learning system $M_\phi$ which can
predict a set of hyper-parameters $\theta'$ based on sensor data $s$
such that, at time step $t_n$, $\theta'_n = M_\phi(s_n)$, and $\theta'_n
= \argmax_{\theta} h(L_\theta)$.



==> dump.tex <==
\subsection{DUMP HERE FOR NOW}

Unlike some other fields, such as computer vision, robot navigation has not settled on a few well estalished benchmarks for evaluating approaches.
Rather, newly proposed approaches are generally compared to one or more widely used or state-of-the-art approaches in a real or simulated navigation task created specifically for that comparison \cite{comparison-rt-oa, ftg}. 

Common metrics for benchmarking approaches include those related to success, safety, and path quality \cite{quantitative-navigation-metrics, nowak2010benchmarks}. 
Attempts have been made at introducing standard benchmarks \cite{Sprunk2016}, often targeted at specific subset such as interactive tasks \cite{interactive-gibson-benchmark} and training learning-based agents \cite{habitat-embodied-ai}.

Some work has been done in benchmarking traditional navigation appraoches against learned ones, though the approaches used were restricted to an action space of only 3 \cite{mishkin2019benchmarking} or 4 \cite{habitat-embodied-ai} discrete actions.



